Asking and Answering Questions to Extract Event-Argument Structures

This paper presents a question-answering approach to extract document-level event-argument structures. We automatically ask and answer questions for each argument type an event may have. Questions are generated using manually defined templates and generative transformers. Template-based questions are generated using predefined role-specific wh-words and event triggers from the context document. Transformer-based questions are generated using large language models trained to formulate questions based on a passage and the expected answer. Additionally, we develop novel data augmentation strategies specialized in inter-sentential event-argument relations. We use a simple span-swapping technique, coreference resolution, and large language models to augment the training instances. Our approach enables transfer learning without any corpora-specific modifications and yields competitive results with the RAMS dataset. It outperforms previous work, and it is especially beneficial to extract arguments that appear in different sentences than the event trigger. We also present detailed quantitative and qualitative analyses shedding light on the most common errors made by our best model.

==> figs/da_gpt3.tex <==
\framebox(4.4in,1.5in){\parbox{4.3in}{
		Secretary of State Hillary Clinton has taken a hard line against Iran's nuclear ambitions, recently thwarting \textcolor{red}{\argsubg{agreements}{event}} tentatively negotiated between the two countries. \textcolor{teal}{\argsubg{Clinton}{violator}} has pushed for punishing sanctions, as she argued that any negotiated settlement was not enough to ensure \textcolor{teal}{\argsubg{Iran}{otherparticipant}} would not pursue nuclear weapons. Her opposition to the agreements was based on Iran's offer to swap its low-enriched uranium for nuclear isotopes, which she felt was not sufficient to prevent their potential proliferation. Iran initially sought to refine the uranium to the levels necessary for energy production, but Clinton insisted that the sanctions remain in place. As the situation between Iran and the United States continues to evolve, Clinton's hard-line stance on the Iranian nuclear issue remains.}}

==> figs/da_lc1.tex <==
\framebox(4.4in,1.5in){\parbox{4.3in}{
		 As Secretary of State, Hillary Clinton was a hawk on the Iranian nuclear issue. In 2009 - 2010, when Iran first indicated a willingness to compromise, \textcolor{teal}{\argsubg{she}{violator}} led the opposition to any negotiated settlement and pushed for punishing sanctions. To clear the route for sanctions, Clinton helped sink \textcolor{red}{\argsubg{agreements}{event}} tentatively negotiated with \textcolor{blue}{\argsubg{Iran}{otherparticipant}} to ship most of its low - enriched uranium out of the country. In 2009, Iran was refining uranium only to the level of about 3-4 percent, as needed for energy production. Its negotiators offered to swap much of that for nuclear isotopes for medical research.}}

==> figs/da_lc2.tex <==
\framebox(4.4in,1.5in){\parbox{4.3in}{
		As Secretary of State, \textcolor{teal}{\argsubg{Hillary Clinton}{violator}} was a hawk on the Iranian nuclear issue. In 2009 - 2010, when Iran first indicated a willingness to compromise, she led the opposition to any negotiated settlement and pushed for punishing sanctions. To clear the route for sanctions, Clinton helped sink \textcolor{red}{\argsubg{agreements}{event}} tentatively negotiated with \textcolor{blue}{\argsubg{Iran}{otherparticipant}} to ship most of its low - enriched uranium out of the country. In 2009, Iran was refining uranium only to the level of about 3-4 percent, as needed for energy production. Its negotiators offered to swap much of that for nuclear isotopes for medical research.}}

==> figs/da_original.tex <==
\framebox(4.2in,1in){}

==> figs/da_pegasus.tex <==
\framebox(4.4in,1.5in){\parbox{4.3in}{
		Hillary Clinton was a strong supporter of the Iranian nuclear issue as Secretary of State. She led the opposition to any negotiated settlement and pushed for punishing sanctions after Iran indicated a willingness to compromise. \textcolor{teal}{\argsubg{Clinton}{violator}} helped sink \textcolor{red}{\argsubg{agreements}{event}} that would have allowed \textcolor{teal}{\argsubg{Iran}{otherparticipant}} to ship most of its low - enriched uranium out of the country. Iran only refined about 3 - 4 percent of its nuclear material in 2009, as needed for energy production. Much of that was offered to be used for medical research.}}

==> figs/da_sw1.tex <==
%\framebox(4.4in,1.5in){\parbox{4.3in}{
\textcolor{teal}{\argsubg{Clinton}{violator}} As Secretary of State, Hillary Clinton was a hawk on the Iranian nuclear issue. In 2009 - 2010, when Iran first indicated a willingness to compromise, she led the opposition to any negotiated settlement and pushed for punishing sanctions. To clear the route for sanctions, helped sink \textcolor{red}{\argsubg{agreements}{event}} tentatively negotiated with \textcolor{blue}{\argsubg{Iran}{otherparticipant}} to ship most of its low - enriched uranium out of the country. In 2009, Iran was refining uranium only to the level of about 3-4 percent, as needed for energy production. Its negotiators offered to swap much of that for nuclear isotopes for medical research.%}%}

==> figs/da_sw2.tex <==
\framebox(4.4in,1.65in){\parbox{4.3in}{
		The violator of the event \textcolor{red}{agreements} is \textcolor{teal}{\argsubg{Clinton}{violator}}. As Secretary of State, Hillary Clinton was a hawk on the Iranian nuclear issue. In 2009 - 2010, when Iran first indicated a willingness to compromise, she led the opposition to any negotiated settlement and pushed for punishing sanctions. To clear the route for sanctions, Clinton helped sink \textcolor{red}{\argsubg{agreements}{event}} tentatively negotiated with \textcolor{blue}{\argsubg{Iran}{otherparticipant}} to ship most of its low - enriched uranium out of the country. In 2009, Iran was refining uranium only to the level of about 3-4 percent, as needed for energy production. Its negotiators offered to swap much of that for nuclear isotopes for medical research.}}

==> figs/rams_example.tex <==
\vspace{1.5in}

==> tex/a_rams.tex <==
\section{RAMS Statistics}
\label{a:rams}


\begin{table}[h!]
\small
\centering
\input{tables/rams_stats}
\caption{Basic statistics of the RAMS dataset.}
\label{t:rams_stats}
\end{table}

Table \ref{t:rams_stats} presents basic statistics of the RAMS dataset.
